Multiuser-MIMO Systems Using Comparator Network-Aided Receivers With 1-Bit Quantization

Low-resolution analog-to-digital converters (ADCs) are promising for reducing energy consumption and costs of multiuser multiple-input multiple-output (MIMO) systems with many antennas. We propose low-resolution multiuser MIMO receivers where the signals are simultaneously processed by 1-bit ADCs and a comparator network, which can be interpreted as additional virtual channels with binary outputs. We distinguish the proposed comparator networks in fully and partially connected. For such receivers, we develop the low-resolution aware linear minimum mean-squared error (LRA-LMMSE) channel estimator and detector according to the Bussgang theorem. We also develop a robust detector which takes into account the channel state information (CSI) mismatch statistics. By exploiting knowledge of the channel coefficients we devise a mean-square error (MSE) greedy search and a sequential signal-to-interference-plus-noise ratio (SINR) search for optimization of partially connected networks. Numerical results show that a system with extra virtual channels can outperform a system with additional receive antennas, in terms of bit error rate (BER). Furthermore, by employing the proposed channel estimation with its error statistics, we construct a lower bound on the ergodic sum rate for a linear receiver. Simulation results confirm that the proposed approach outperforms the conventional 1-bit MIMO system in terms of BER, MSE and sum rate.

==> Linear_Detection/Robust_Detection_channel_estimation_error.tex <==
\subsection{Robust LRA-LMMSE Detector for Imperfect CSI Caused by Channel Estimation}
\label{sec:Robust_1}
In this subsection, a robust LRA-MMSE detector is proposed, which takes the channel estimation and its corresponding error statistics into account. In this context, based on the channel estimation error  $\bm{\varepsilon}_{\text{R}} = \mathbf{h}_{\text{R}} -\hat{\mathbf{h}}_{\text{R, LRA-LMMSE}} $, we redefine the received signal as
\begin{equation}
\begin{split}
\mathbf{y}_{\text{R}_r} &= \begin{bmatrix} 
\mathfrak{R}\{\tilde{\mathbf{X}}\} &-\mathfrak{I}\{\tilde{\mathbf{X}}\}\\
\mathfrak{I}\{\tilde{\mathbf{X}}\} & \mathfrak{R}\{\tilde{\mathbf{X}}\}
\end{bmatrix}\begin{bmatrix}
\mathfrak{R}\{\mathbf{h}\} \\
\mathfrak{I}\{\mathbf{h}\}
\end{bmatrix} +
\begin{bmatrix}
\mathfrak{R}\{\mathbf{n}_{d}\} \\
\mathfrak{I}\{\mathbf{n}_{d}\}
\end{bmatrix}\\
%&= \tilde{\mathbf{X}}_{\text{R}}\mathbf{h}_{\text{R}} +\mathbf{n}_{{\text{R}}_d}= \tilde{\mathbf{X}}_{\text{R}}\left(\hat{\mathbf{h}}_{\text{R, LRA-LMMSE}} + \bm{\varepsilon}_{\text{R}}\right) +\mathbf{n}_{{\text{R}}_d} \\
&= \hat{\mathbf{H}}_{\text{R}}\mathbf{x}_{\text{R}} + \tilde{\mathbf{X}}_{\text{R}}\bm{\varepsilon}_{\text{R}} +\mathbf{n}_{{\text{R}}_d},
\end{split}
\end{equation}
where $\mathbf{y}_{\text{R}_r} \in \mathbb{R}^{2 N_r \times 1} $ and $\tilde{\mathbf{X}} = (\mathbf{x}^T\otimes\mathbf{I}_{N_r}) \in \mathbb{C}^{N_r \times N_t N_r}$. The subscript $d$  refers to data. Moreover, $\hat{\mathbf{H}}_{\text{R}} \in \mathbb{R}^{2 N_r \times 2 N_t}$ is the estimated channel matrix described by
\begin{equation}
\begin{split}
&\hat{\mathbf{H}}_{\text{R}} =  \begin{bmatrix} 
\mathfrak{R}\{\hat{\mathbf{H}}\} &-\mathfrak{I}\{\hat{\mathbf{H}}\}\\
\mathfrak{I}\{\hat{\mathbf{H}}\} & \mathfrak{R}\{\hat{\mathbf{H}}\}
\end{bmatrix}  \text{with} \enspace \hat{\mathbf{H}} = \text{unvec}(\hat{\mathbf{h}}) \\
&\text{and} \enspace \hat{\mathbf{h}} = \begin{bmatrix}
\hat{\mathbf{h}}_{\text{R, LRA-LMMSE, a}}  + j\hat{\mathbf{h}}_{\text{R, LRA-LMMSE, b}}
\end{bmatrix},
\label{eq:H_hat}
\end{split}
\end{equation}
where $\hat{\mathbf{h}}_{\text{R, LRA-LMMSE, a}}$ corresponds to the first half of the estimated channel $\hat{\mathbf{h}}_{\text{R, LRA-LMMSE}}$ and $\hat{\mathbf{h}}_{\text{R, LRA-LMMSE, b}}$ to the second, as shown in \eqref{eq:h_estimated}. Therefore, the quantized signal for the robust detector is given by
\begin{equation}
\begin{split}
\mathbf{z}_{\mathcal{Q}_r} &= \mathcal{Q} (\mathbf{z}_{{\text{R}}_r}) = \mathbf{A}_{{\text{R}}_r} \mathbf{B}\hat{\mathbf{H}}_{\text{R}} \mathbf{x}_{\text{R}} + \mathbf{A}_{{\text{R}}_r} \mathbf{B} \tilde{\mathbf{X}}_{\text{R}}\bm{\varepsilon}_{\text{R}}  + \mathbf{A}_{{\text{R}}_r} \mathbf{B} \mathbf{n}_{{\text{R}}_d} + \mathbf{n}_{{\text{R}}_{q, d}},
\end{split}
\end{equation}
where $\mathbf{A}_{{\text{R}}_r}$ is the Bussgang-based linear operator for the transmit data, similarly as calculated in \eqref{eq:A_rp}. Then, the linear LRA-LMMSE filter is applied to $\mathbf{z}_{\mathcal{Q}_r}$, to obtain
\begin{equation}
\hat{\mathbf{x}}_{\text{R}} =\mathbf{G}_{\text{R}}^T \mathbf{z}_{\mathcal{Q}_r},
\end{equation}
where the matrix $\mathbf{G}_{\text{R}}$
is chosen to minimize the MSE between the transmitted symbol $\mathbf{x}_{\text{R}}$
and the filter output, i.e.,
\begin{equation}
\begin{split}
\tilde{\mathbf{G}}_{\text{R, LRA-MMSE}} &= \arg\min_{\mathbf{G}_{\text{R}}}\enspace E\left[\left\vert\left\vert \mathbf{x}_{\text{R}}-\mathbf{G}_{\text{R}}^T\mathbf{z}_{\mathcal{Q}_r}\right\vert\right\vert^2_2\right]\\
&= \arg\min_{\mathbf{G}_{\text{R}}}\enspace -2\mathrm{tr} \left(\mathbf{G}_{\text{R}}^T \mathbf{C}_{\mathbf{z}_{\mathcal{Q}_r}\mathbf{x}_{\text{R}}} \right) + \mathrm{tr} \left(\mathbf{G}_{\text{R}}^T\mathbf{C}_{\mathbf{z}_{\mathcal{Q}_r}}\mathbf{G}_{\text{R}} \right),
\label{eq:G_LRAMMSE_2}
\end{split}
\end{equation}
where the latter describes an equivalent problem.
%\emph{Derivation}: See Appendix \ref{subsec:derivation_of_G_LRAMMSE_2}.

By differentiating \eqref{eq:G_LRAMMSE_2} with respect to $\mathbf{G}_{\text{R}}^T$ and equating it to zero, the solution of the LRA-LMMSE
receive filter is given by
\begin{equation}
\tilde{\mathbf{G}}_{\text{R, LRA-MMSE}} = \mathbf{C}_{\mathbf{z}_{\mathcal{Q}_r}}^{-1}\mathbf{C}_{\mathbf{z}_{\mathcal{Q}_r}\mathbf{x}_{\text{R}}}.
\label{eq:Robust_G}
\end{equation}
As in the previous cases, the covariance matrix is calculated as \cite{Jacovitti}
\begin{equation}
\mathbf{C}_{\mathbf{z}_{\mathcal{Q}_r}} = \frac{2}{\pi}\text{sin}^{-1}\left(\mathbf{K}_{\text{R}_r}\mathbf{C}_{\mathbf{z}_{\text{R}_r}}\mathbf{K}_{\text{R}_r}\right),
\end{equation}
and the cross-correlation matrix is based on the Bussgang theorem \cite{Bussgang}
\begin{equation}
\mathbf{C}_{\mathbf{z}_{\mathcal{Q}_r}\mathbf{x}_{\text{R}}} = \sqrt{\frac{2}{\pi}}\frac{1}{2}\mathbf{K}_{\text{R}_r} \mathbf{B} \hat{\mathbf{H}}_{\text{R}},
\label{eq:Czqxr_2}
\end{equation}
with $\mathbf{K}_{\text{R}_r}=\text{diag}(\mathbf{C}_{\mathbf{z}_{\text{R}_r}})^{-\frac{1}{2}}$ and the cross-correlation matrix between $\mathbf{z}_{\text{R}_r}$ and $\mathbf{x}_{\text{R}}$ is given by
\begin{equation}
\mathbf{C}_{\mathbf{z}_{\text{R}_r}\mathbf{x}_{\text{R}}} = \frac{1}{2} \mathbf{B}\hat{\mathbf{H}}_{\text{R}},    
\end{equation}
where due to the real-valued notation of the system the input correlation matrix $\mathbf{C_{\mathbf{x}_{\text{R}}}} = E\left[\mathbf{x}_{\text{R}}\mathbf{x}_{\text{R}}^T\right] =\frac{1}{2}\mathbf{I}_{2N_t}$ is considered.\\
%\emph{Derivation}: See Appendix \ref{subsec:derivation_of_Czqxr2}.

Moreover, the correlation matrix of the unquantized output signal $\mathbf{z}_{\text{R}_r}$ is given by
\begin{equation}
\begin{split}
\mathbf{C}_{\mathbf{z}_{\text{R}_r}} = \frac{1}{2}\mathbf{B}\hat{\mathbf{H}}_{\text{R}}\hat{\mathbf{H}}_{\text{R}}^T\mathbf{B}^T + \mathbf{B}\mathbf{\Gamma}_{{\text{R}}}\mathbf{B}^T + \frac{\sigma_n^2}{2}\mathbf{B}\mathbf{B}^T.
\label{eq:Czr_2}
\end{split}
\end{equation}
%\emph{Derivation}: See Appendix \ref{subsec:derivation_of_Czr2}.

The matrix  $\mathbf{\Gamma}_{{\text{R}}}$ in \eqref{eq:Czr_2} is calculated as follows
\begin{equation}
\begin{split}
\mathbf{\Gamma}_{{\text{R}}} &= E\left[\tilde{\mathbf{X}}_{\text{R}}E\left[\bm{\varepsilon}_{\text{R}}\bm{\varepsilon}_{\text{R}}^T\right]\tilde{\mathbf{X}}_{\text{R}}^T\right]
= E\left[\tilde{\mathbf{X}}_{\text{R}}\mathbf{R_{h_{\text{R}}}}\tilde{\mathbf{X}}_{\text{R}}^T -\tilde{\mathbf{X}}_{\text{R}}\mathbf{R_{h_{\text{R}}}}\hat{\mathbf{\Phi}}_{\text{R}}^T  \mathbf{C}_{\mathbf{z}_{\mathcal{Q}_{p}}}^{-1}\hat{\mathbf{\Phi}}_{\text{R}} \mathbf{R_{h_{\text{R}}}} \tilde{\mathbf{X}}_{\text{R}}^T\right],
\label{eq:gamma_r}
\end{split}
\end{equation}
where $E\left[\bm{\varepsilon}_{\text{R}}\bm{\varepsilon}_{\text{R}}^T\right] = \mathbf{R_{h_{\text{R}}}} -\mathbf{R_{h_{\text{R}}}}\hat{\mathbf{\Phi}}_{\text{R}}^T  \mathbf{C}_{\mathbf{z}_{\mathcal{Q}_{p}}}^{-1}\hat{\mathbf{\Phi}}_{\text{R}} \mathbf{R_{h_{\text{R}}}}$, similarly as previously calculated in \eqref{eq:mse}. 
In the following it is considered that the transmit symbols are taken from an $M_x$-ary symbol alphabet and that the prior probabilities are known at the receiver. 
With this, the expected value in \eqref{eq:gamma_r} can be calculated as
\begin{equation}
\begin{split}
\mathbf{\Gamma}_{{\text{R}}} &= \sum_{i = 1}^{M_x^{N_t}} P\left( \tilde{\mathbf{X}}_{\text{R}, i} \right) \left(\tilde{\mathbf{X}}_{\text{R}, i}\mathbf{R_{h_{\text{R}}}}\tilde{\mathbf{X}}_{\text{R}, i}^T -\tilde{\mathbf{X}}_{\text{R}, i}\mathbf{R_{h_{\text{R}}}}\hat{\mathbf{\Phi}}_{\text{R}}^T  \mathbf{C}_{\mathbf{z}_{\mathcal{Q}_{p}}}^{-1}\hat{\mathbf{\Phi}}_{\text{R}} \mathbf{R_{h_{\text{R}}}} \tilde{\mathbf{X}}_{\text{R}, i}^T \right) \text{.}
\end{split}
\end{equation}
Considering that the transmit symbols are uniformly distributed QPSK symbols the computation simplifies to
\begin{equation}
\begin{split}
\mathbf{\Gamma}_{{\text{R}}} &= \frac{1}{4^{N_t}} \sum_{i = 1}^{4^{N_t}} \left(\tilde{\mathbf{X}}_{\text{R}, i}\mathbf{R_{h_{\text{R}}}}\tilde{\mathbf{X}}_{\text{R}, i}^T -\tilde{\mathbf{X}}_{\text{R}, i}\mathbf{R_{h_{\text{R}}}}\hat{\mathbf{\Phi}}_{\text{R}}^T  \mathbf{C}_{\mathbf{z}_{\mathcal{Q}_{p}}}^{-1}\hat{\mathbf{\Phi}}_{\text{R}} \mathbf{R_{h_{\text{R}}}} \tilde{\mathbf{X}}_{\text{R}, i}^T \right).
\end{split}
\end{equation}


==> Linear_Detection/Robust_Detection_extra_part.tex <==
\subsection{Robust LRA-LMMSE Detector for Partially Outdated CSI}
\label{sec:Robust_2}
In this subsection, a detector is developed for partially outdated CSI. In this context, it is considered that the channel can be described by two uncorrelated terms as  
$\mathbf{h}_{\text{R}}  =   \sqrt{\lambda} \hat{\mathbf{h}}_{\text{R}}    + \sqrt{1 - \lambda}  \mathbf{h}_{\text{R, new}}   $, where $\hat{\mathbf{h}}_{\text{R}}, \lambda $ 
and the channel correlation matrices  $ \mathbf{R_{\hat{h}_{\text{R}}}} =  \mathbf{R_{h_{\text{R, new}}}} = \mathbf{R_{h_{\text{R}}}}   $
are considered to be known at the receiver. The quality of the CSI is determined by parameter $0<\lambda<1$.
Then the received signals at the antennas read as  
\begin{align}
    \mathbf{y}_{\text{R}_r} = \sqrt{\lambda}  \hat{\mathbf{H}}_{\text{R}}\mathbf{x}_{\text{R}} +
    \sqrt{1 - \lambda}
    \tilde{\mathbf{X}}_{\text{R}}\mathbf{h}_{\text{R, new}} +\mathbf{n}_{{\text{R}}_d} \text{.}
\end{align}
Moreover, the linear model for the outputs of the ADCs and comparator network is given by
\begin{align}
    \mathbf{z}_{\mathcal{Q}_r} &= \mathcal{Q} (\mathbf{z}_{{\text{R}}_r}) =   
    \sqrt{\lambda} 
    \mathbf{A}_{{\text{R}}_r} \mathbf{B}\hat{\mathbf{H}}_{\text{R}} \mathbf{x}_{\text{R}} + 
      \sqrt{1 - \lambda}
    \mathbf{A}_{{\text{R}}_r} \mathbf{B} \tilde{\mathbf{X}}_{\text{R}}\mathbf{h}_{\text{R, new}}  + \mathbf{A}_{{\text{R}}_r} \mathbf{B} \mathbf{n}_{{\text{R}}_d} + \mathbf{n}_{{\text{R}}_{q, d}} \text{.}
\end{align}
The corresponding robust detector has the same form as \eqref{eq:Robust_G} and for brevity only the different terms are described below.
The channel input-output cross correlation function reads as 
\begin{align}
\mathbf{C}_{\mathbf{z}_{\mathcal{Q}_r}\mathbf{x}_{\text{R}}} = \sqrt{\frac{ 2 \lambda }{\pi}}\frac{1}{2}\mathbf{K}_{\text{R}_r} \mathbf{B} \hat{\mathbf{H}}_{\text{R}}.   
\end{align}
Moreover, correlation matrix of the unquantized virtual channel is given by
\begin{align}
\mathbf{C}_{\mathbf{z}_{\text{R}_r}} = \frac{\lambda}{2}\mathbf{B}\hat{\mathbf{H}}_{\text{R}}\hat{\mathbf{H}}_{\text{R}}^T\mathbf{B}^T + (1-\lambda)  \mathbf{B}
E\left[\tilde{\mathbf{X}}_{\text{R}}\mathbf{R_{h_{\text{R}}}}\tilde{\mathbf{X}}_{\text{R}}^T \right]
\mathbf{B}^T + \frac{\sigma_n^2}{2}\mathbf{B}\mathbf{B}^T.
\end{align}



==> Numerical_results/BER_Comparison.tex <==
\subsection{Linear Detection}
\label{subsec:ber_comparisons}

\subsubsection{Proposed LRA-LMMSE Detector}
$\\$
In this subsection, it is considered a system with $N_r = 10$. While making the signal detection, the LRA-MMSE detector is applied in the system. The BER performance plots are obtained by taking the average of $2000$ different channels and $2000$ noise realizations per channel.

\begin{figure}[ht]
\centering
\input{figures/BER_2x10all}
\caption{BER performance of LRA-LMMSE detectors with and without comparator network in $2\times10$ MIMO systems.}
\label{fig:BER2x10all}    
\end{figure}

The LRA-LMMSE detector BER performance of fully and partially connected networks under perfect CSI are shown in Fig. \ref{fig:BER2x10all}. The partially connected cases refers to $\alpha_p=20$ comparators, while the case of fully connected networks refers to $\alpha_f=190$ comparators.

Simulation results shows that the system with fully connected network achieves the best BER performance with the cost of a large number of comparators. In the partially connected networks, the MMSE based greedy search outperforms the random selection approach especially at high SNR, where the error floor is eliminated. A surprising observation is that the greedy search approach has almost the same BER performance as the fully connected method but with much less comparators. This shows great advantages of the greedy search based partially connected network. However, also the approach with the comparator network using random selected inputs is beneficial in terms of BER. While making comparison with the approach without additional comparator network, it can be seen that by adding extra $20$ comparators the performance gain is significant and the error floor goes down largely.

However, it should be mentioned that although the greedy search approach yields comparable good BER performance and less usage of the comparators, the computational cost is the highest among the approaches due to its iterative search for the least MSE values.



\vspace{1em}
\subsubsection{Robust LRA-LMMSE Detector}
$\\$
In this subsection, it is considered a system with $N_r=4$. The BER performance plots are obtained by taking the average of $1000$ different channels and $1000$ noise realizations per channel.

\begin{figure}[ht]
\centering
\input{figures/BER_2x4_ROBUST}
\caption{BER comparisons of LRA-LMMSE detectors with and without comparator network in $2\times4$ MIMO systems.} 
\label{fig:BER_2x4_ROBUST}    
\end{figure}

\begin{figure}[ht!]
\centering
\input{figures/MSE_2x4_ROBUST}
\caption{MSE comparisons of LRA-LMMSE detectors with and without comparator network in $2\times4$ MIMO systems.} 
\label{fig:MSE_2x4_ROBUST}    
\end{figure}

The robust LRA-LMMSE detector BER performance of fully and partially connected networks is illustrated in Fig. \ref{fig:BER_2x4_ROBUST}. In this experiment, the partially connected networks have $\alpha_p=8$ comparators, while the fully connected have $\alpha_f=28$ comparators. The LRA-LMMSE detector is based on the channel estimate while the Robust LRA-LMMSE detector combines the proposed channel estimate with the corresponding estimation error. As expected, simulation results shows that the Robust LRA-LMMSE detector obtain an advantage in comparison to the non-robust one. This benefit is not only in terms of BER but also MSE as shown in Fig. \ref{fig:MSE_2x4_ROBUST}.  

==> Numerical_results/MSE_Comparison.tex <==
\subsection{Channel Estimation}
\label{subsec:mse_comparisons}

In this subsection, it is considered a system with $N_r=4$. The presented performance plots are obtained by taking the average of $2000$ different channels and $2000$ noise realizations per channel. Moreover, the lines labeled as ``Analytical Result'' are obtained with (\ref{eq:mse}) while the marks labeled as ``Numerical Result'' are obtained with the MSE of the simulated channel estimator in (\ref{eq:h_estimated}).

\begin{figure}[ht]
\centering
\input{figures/MSE_2x4}
\caption{MSE comparisons of LRA-LMMSE channel estimators  with and without comparator network in $2\times4$ MIMO systems with $\tau= N_t$.} 
\label{fig:MSE_2x4}    
\end{figure}


The MSE comparison between the LRA-LMMSE channel estimators with fully and partially connected comparator networks are shown in Fig. \ref{fig:MSE_2x4}. The numerical and analytical results are aligned, which confirms the accuracy of the proposed model. As expected, the  system with the fully connected method  achieves  the  best MSE performance. However, it can be seen that the approach  with the comparator network using random selected inputs is also beneficial in terms of MSE in comparison to the case without comparator network. 




==> Numerical_results/Sum_Rate_Comparison.tex <==
\subsection{Sum Rate Analysis}
\label{subsec:sum_rate_comparisons}

In this section, it is considered a system with $N_r=4$. The Sum Rate plots are obtained by taking the average of $2000$ different channels and $2000$ noise realizations per channel.

\begin{figure}[ht]
\centering
\input{figures/AR_2x4}
\caption{Sum Rate comparisons of LRA-LMMSE channel estimators  with and without comparator network in $2\times4$ MIMO systems.} 
\label{fig:AR_2x4}    
\end{figure}

The comparison between the lower bound of the ergodic sum rate with and without the comparator network is presented. The sum rate versus SNR for the systems is shown in Fig. \ref{fig:AR_2x4}, which indicates a significant benefit for the system that utilizes the additional comparator networks. We can see that the system with fully connected network achieves the best sum rate performance, followed by the MMSE based greedy search and the random selected inputs. Note that the increased sum rate is not only due to a more accurate channel estimation but also due to the comparator network aided receive processing.

==> Sum_Rate/MF_Sum_Rate.tex <==
\textcolor{green}{
\subsection{Sum Rate for Matched Filter Receiver}
The corresponding matched filter for the $k$th substream for the system with comparator network can be expressed as  
$\mathbf{g}_{\text{R}_{k}}^T=\hat{\mathbf{h}}_{\text{R}_{k}}^T \mathbf{B}^T \mathbf{A}_{{\text{R}}_d}^T$, with
$\mathbf{A}_{{\text{R}}_d}=\sqrt{\frac{2}{\pi}} \mathrm{diag}(\mathbf{C}_{\mathbf{z}_{{\text{R}}_d}})^{-\frac{1}{2}}$
\begin{align}
\mathrm{E}[\mathbf{A}_{{\text{R}}_d}]=
\sqrt{\frac{2}{\pi}} \mathrm{diag}  \left(   \mathrm{E}\left[
\frac{\sigma_x^2}{2}\mathbf{BH}_{\text{R}}{\mathbf{H}_{\text{R}}^T}\mathbf{B}^T+\frac{\sigma_n^2}{2}\mathbf{BB}^T \right]
\right)  ^{-\frac{1}{2}}
\end{align}
Considering a generic channel with $\mathrm{E}[\mathbf{H}_{\text{R}}{\mathbf{H}_{\text{R}}^T}]= N_t \mathbf{I} $
\begin{align}
\mathrm{E}[\mathbf{A}_{{\text{R}}_d}]=
\sqrt{\frac{2}{\pi} \frac{2}{N_t \sigma_x^2+\sigma_n^2}}
\mathbf{I}_{2 N_r +\alpha} \text{.}
\label{eq:Bussgang_Operator_data}
\end{align}
In the following, the prefactor in \eqref{eq:Bussgang_Operator_data} is termed $\zeta$.
The received signal after filtering can be expressed alternatively as
\begin{align}
\hat{\mathbf{x}}_{\text{R}_{k}} = \quad & \mathrm{E} [  \mathbf{g}_{\text{R}_{k}}^T \mathbf{A}_{{\text{R}}_d} \mathbf{B} {\mathbf{h}}_{\text{R}_{k}}]\mathbf{x}_{\text{R}_{k}} + n_{\text{eff},k} \text{,}
\end{align}
where $n_{\text{eff},k}$ represents some effective noise term.
For the matched filtering approach under the mentioned assumptions it holds
\begin{align}
\mathrm{E} [  \mathbf{g}_{\text{R}_{k}}^T \mathbf{A}_{{\text{R}}_d} \mathbf{B} {\mathbf{h}}_{\text{R}_{k}}] = 
\zeta^2
\mathrm{E} [  \hat{\mathbf{h}}_{\text{R}_{k}}^T \mathbf{B}^T
\mathbf{B}  \hat{\mathbf{h}}_{\text{R}_{k}}
]
\text{.}
\end{align}
In the next step it is considered that $\mathbf{B}^T
\mathbf{B}$ can be approximated by $(1+\frac{\alpha}{2 N_r}) \mathbf{I}$
\begin{align}
\mathrm{E} [  \mathbf{g}_{\text{R}_{k}}^T \mathbf{A}_{{\text{R}}_d} \mathbf{B} {\mathbf{h}}_{\text{R}_{k}}] = 
\zeta^2
\left(1+\frac{\alpha}{2 N_r}\right)
 \mathrm{trace} [  \mathrm{E} [   \hat{\mathbf{h}}_{\text{R}_{k}}
\hat{\mathbf{h}}_{\text{R}_{k}}^T  ]  ]
\text{.}
\end{align}
From \eqref{eq:correlation_estimation} it follows
\begin{align}
\mathrm{E} [  \mathbf{g}_{\text{R}_{k}}^T \mathbf{A}_{{\text{R}}_d} \mathbf{B} {\mathbf{h}}_{\text{R}_{k}}] = 
\zeta^2
\left(1+\frac{\alpha}{2 N_r}\right)
2N_r \kappa
\label{eq:MF_exp_value}
\text{.}
\end{align}
The corresponding variance is given by
\begin{align}
\mathrm{Var} [  \mathbf{g}_{\text{R}_{k}}^T \mathbf{A}_{{\text{R}}_d} \mathbf{B} {\mathbf{h}}_{\text{R}_{k}}]=
\mathrm{E} [  \mathbf{g}_{\text{R}_{k}}^T \mathbf{A}_{{\text{R}}_d} \mathbf{B} {\mathbf{h}}_{\text{R}_{k}}
{\mathbf{h}}_{\text{R}_{k}}^T
\mathbf{B}^T
\mathbf{A}_{{\text{R}}_d}^T
\mathbf{g}_{\text{R}_{k}}
]-\mathrm{E} [  \mathbf{g}_{\text{R}_{k}}^T \mathbf{A}_{{\text{R}}_d} \mathbf{B} {\mathbf{h}}_{\text{R}_{k}}]^2 \text{.}
\end{align}
By considering $\mathbf{B}^T
\mathbf{B}=(1+\frac{\alpha}{2N_r}) \mathbf{I} $ the variance can be rewritten as
\begin{align}
\mathrm{Var} [  \mathbf{g}_{\text{R}_{k}}^T \mathbf{A}_{{\text{R}}_d} \mathbf{B} {\mathbf{h}}_{\text{R}_{k}}]=
\zeta^4
\left(   1+\frac{\alpha}{2 N_r}  \right)^2
\mathrm{E} [    | \hat{\mathbf{h}}_{\text{R}_{k}}^T  {\mathbf{h}}_{\text{R}_{k}}   |^2
]-\mathrm{E} [  \mathbf{g}_{\text{R}_{k}}^T \mathbf{A}_{{\text{R}}_d} \mathbf{B} {\mathbf{h}}_{\text{R}_{k}}]^2  \text{,}
\end{align}
which can be expressed as
\begin{align}
& \mathrm{Var} [  \mathbf{g}_{\text{R}_{k}}^T \mathbf{A}_{{\text{R}}_d} \mathbf{B} {\mathbf{h}}_{\text{R}_{k}}]=  \\
& \zeta^4
\left(   1+\frac{\alpha}{2 N_r}  \right)^2
\left(
\mathrm{E} [     \hat{\mathbf{h}}_{\text{R}_{k}}^T  {\mathbf{h}}_{\text{R}_{k}}   
]^2
+
\mathrm{Var} [     \hat{\mathbf{h}}_{\text{R}_{k}}^T  {\mathbf{h}}_{\text{R}_{k}}  
]
\right)
-\mathrm{E} [  \mathbf{g}_{\text{R}_{k}}^T \mathbf{A}_{{\text{R}}_d} \mathbf{B} {\mathbf{h}}_{\text{R}_{k}}]^2  \text{.} \notag
\end{align}
By considering $\mathrm{E} [     \hat{\mathbf{h}}_{\text{R}_{k}}^T  {\mathbf{h}}_{\text{R}_{k}}   
] =  \mathrm{E} [     \hat{\mathbf{h}}_{\text{R}_{k}}^T   \hat{{\mathbf{h}}}_{\text{R}_{k}}   
]   $ and \eqref{eq:MF_exp_value} the variance reduces to
\begin{align}
\mathrm{Var} [  \mathbf{g}_{\text{R}_{k}}^T \mathbf{A}_{{\text{R}}_d} \mathbf{B} {\mathbf{h}}_{\text{R}_{k}}]=  
 \zeta^4
\left(   1+\frac{\alpha}{2 N_r}  \right)^2
\left(
\mathrm{Var} [     \hat{\mathbf{h}}_{\text{R}_{k}}^T  \hat{\mathbf{h}}_{\text{R}_{k}}  
]
+
\mathrm{Var} [     \hat{\mathbf{h}}_{\text{R}_{k}}^T  {\mathbf{\epsilon}}_{\text{R}_{k}}   
]
\right)
\end{align}
Considering that the entries in $\hat{\mathbf{h}}_{\text{R}_{k}} $ are Gaussian distributed, it follows that $\|  \hat{\mathbf{h}}_{\text{R}_{k}} \|^2$ is chi squared distributed with $2N_r$ degrees of freedom and $ \mathrm{E}[ \|  \hat{\mathbf{h}}_{\text{R}_{k}} \|^2]= 2 N_r \kappa$ and $ \mathrm{Var}[ \|  \hat{\mathbf{h}}_{\text{R}_{k}} \|^2]= 4 N_r \kappa^2$. 
Considering that the entries in
${\mathbf{\epsilon}}_{\text{R}_{k}}$ are uncorrelated with the channel estimate and Gaussian distributed, 
the variance is given by
\begin{align}
\mathrm{Var} [  \mathbf{g}_{\text{R}_{k}}^T \mathbf{A}_{{\text{R}}_d} \mathbf{B} {\mathbf{h}}_{\text{R}_{k}}]=  
 \zeta^4
\left(   1+\frac{\alpha}{2 N_r}  \right)^2
\left(
4 N_r \kappa^2
+
N_r \kappa(1-2\kappa)
\right)
\end{align}
This finally yields
\begin{align}
\mathrm{Var}[  \mathbf{g}_{\text{R}_{k}}^T \mathbf{A}_{{\text{R}}_d} \mathbf{B} {\mathbf{h}}_{\text{R}_{k}}]=
\zeta^4
\left(   1+\frac{\alpha}{2 N_r}  \right)^2
N_r \kappa    (2 \kappa  +1     )   \text{.}
\end{align}
The interference variance from the $i$th signal stream can be expressed as
\begin{align}
\mathrm{E}[ |
\mathbf{g}_{\text{R}_{k}}^T\mathbf{A}_{{\text{R}}_d} \mathbf{B} {\mathbf{h}}_{\text{R}_i}\mathbf{x}_{\text{R}_i}   |^2 ] =
\frac{\sigma_x^2}{2}
\zeta^4
\mathrm{E}[ |
\hat{\mathbf{h}}_{\text{R}_{k}}^T      \mathbf{B}^T\mathbf{B} {\mathbf{h}}_{\text{R}_i}   |^2 ] 
 \text{.}
\end{align}
Considering that $\hat{\mathbf{h}}_{\text{R}_{k}}$ and ${\mathbf{h}}_{\text{R}_i}$ are independent yields
\begin{align}
\mathrm{E}[ |
\mathbf{g}_{\text{R}_{k}}^T\mathbf{A}_{{\text{R}}_d} \mathbf{B} {\mathbf{h}}_{\text{R}_i}\mathbf{x}_{\text{R}_i}   |^2 ] =
\frac{\sigma_x^2}{4}
\zeta^4
\mathrm{E}[ |
\hat{\mathbf{h}}_{\text{R}_{k}}^T      \mathbf{B}^T\mathbf{B}   |^2 ] 
 \text{.}
\end{align}
By assuming that the entries in $\mathbf{B}'$ are binary distributed independent variables, the following approximation holds $E[ \mathbf{B}^T  \mathbf{B}
\mathbf{B}^T \mathbf{B}
   ]= E[\mathbf{B}^T
\mathbf{B}]^2+  \mathrm{Cov}[\mathbf{B}^T \mathbf{B}]  \approx  (1+\frac{\alpha}{2N_r})^2  \mathrm{I}  +\frac{\alpha}{4 N_r^2}(N_r-1) \mathrm{I}=\delta_B \mathrm{I}$.
With this, the interference variance reads as
\begin{align}
\mathrm{E}[ |
\mathbf{g}_{\text{R}_{k}}^T\mathbf{A}_{{\text{R}}_d} \mathbf{B} {\mathbf{h}}_{\text{R}_i}\mathbf{x}_{\text{R}_i}   |^2 ] =
\frac{\sigma_x^2}{2}
\zeta^4 \delta_B
N_r \kappa  
 \text{.}
\end{align}
The correlation matrix of the quantization noise is described by
\begin{align}
\mathbf{C}_{\mathbf{n}_{{\text{R}}_{q, d}}} = 
\frac{  \pi-2 }{\pi }
\left( \frac{2}{\pi-2}
\mathbf{B}
\mathbf{B}^T+  \mathbf{I}
\right)
- \zeta^2
\frac{ N_t \sigma_x^2+\sigma_n^2}{2}
\mathbf{B}
\mathbf{B} ^T  \text{.}
\end{align}
This can be expressed as
\begin{align}
\mathbf{C}_{\mathbf{n}_{{\text{R}}_{q, d}}} = 
\frac{  \pi-2 }{\pi }
\mathbf{I}
+
\left(
\frac{2}{\pi}
- \zeta^2
\frac{ N_t \sigma_x^2+\sigma_n^2}{2}   \right)
\mathbf{B}
\mathbf{B} ^T  \text{.}
\end{align}
The quantization noise variance is determined by
\begin{align}
\mathrm{E} [\mathbf{g}_{\text{R}_{k}}^T
\mathbf{C}_{\mathbf{n}_{{\text{R}}_{q, d}}} \mathbf{g}_{\text{R}_{k}}
]
= 
\frac{  \pi-2 }{\pi }
\mathrm{E} [\mathbf{g}_{\text{R}_{k}}^T
 \mathbf{g}_{\text{R}_{k}}
]
+
\left(
\frac{2}{\pi}
- \zeta^2
\frac{ N_t \sigma_x^2+\sigma_n^2}{2}   \right)
\mathrm{E} [\mathbf{g}_{\text{R}_{k}}^T \mathbf{B}
\mathbf{B}^T
 \mathbf{g}_{\text{R}_{k}}
]
  \text{.}
\end{align}
This can be expressed as
\begin{align}
\mathrm{E} [\mathbf{g}_{\text{R}_{k}}^T
\mathbf{C}_{\mathbf{n}_{{\text{R}}_{q, d}}} \mathbf{g}_{\text{R}_{k}}
]
= 
\frac{  \pi-2 }{\pi } \zeta^2 \left(1+\frac{\alpha}{2N_r}  \right)2N_r \kappa   
+ \zeta^2 \delta_B
\left(
\frac{2}{\pi}
- \zeta^2
\frac{ N_t \sigma_x^2+\sigma_n^2}{2}   \right)
2N_r \kappa
  \text{.}
\end{align}
The variance of the thermal noise is given by
\begin{align}
    \mathrm{E} [  \mathbf{g}_{\text{R}_{k}}^T   \mathbf{A}_{{\text{R}}_d} \mathbf{B}
\mathbf{C}_{\mathbf{n}_{{\text{R}}_{d}}}   \mathbf{B}^T \mathbf{A}_{{\text{R}}_d}^T \mathbf{g}_{\text{R}_{k}}   ]  =  \frac{\sigma_n^2}{2} \zeta^4  \delta_B 2N_r \kappa
   \text{.}
\end{align}
The resulting rate per real valued substream is given by
\begin{equation}
\scalebox{0.99}{$
I_{\text{R}_{k}} =  
\frac{1}{2} \log_2 \left ( 1 +  \frac{   \frac{ \sigma_x^2}{2} \zeta^4 \left(1+\frac{\alpha}{2 N_r}\right)^2 4N_r^2 \kappa^2}
{ \frac{\sigma_x^2}{2} \zeta^4
\delta_B
 N_r  \kappa (K-1)
+  \frac{ \sigma_x^2}{2} 
\zeta^4
\left(   1+\frac{\alpha}{2 N_r}  \right)^2
N_r \kappa    (2 \kappa  +1     )
+
\frac{\sigma_n^2}{2} \zeta^4  \delta_B 2N_r \kappa
+
\frac{  \pi-2 }{\pi } \zeta^2 (1+\frac{\alpha}{2N_r})2N_r \kappa 
+ \zeta^2 \delta_B
\left(
\frac{2}{\pi}
- \zeta^2
\frac{ N_t \sigma_x^2+\sigma_n^2}{2}   \right)
2N_r \kappa}
\right)   
$}    \text{.}   \notag 
\label{eq:I_analytical}
\end{equation}
This can be written more compact as
\begin{equation}
\scalebox{0.99}{$
I_{\text{R}_{k}} = 
\frac{1}{2} \log_2 \left ( 1 +  \frac{  \sigma_x^2 
\left(1+\frac{\alpha}{2 N_r}\right)^2
2N_r \kappa
}{ \frac{\sigma_x^2}{2}
\delta_B
    (K-1)
+  \frac{ \sigma_x^2}{2} 
\left(   1+\frac{\alpha}{2 N_r}  \right)^2
     (2 \kappa  +1     )
+
\sigma_n^2 \delta_B 
+
2\frac{  \pi-2 }{\pi } \zeta^{-2} (1+\frac{\alpha}{2N_r})    
+ 2 \zeta^{-2} \delta_B
\left(
\frac{2}{\pi}
- \zeta^2
\frac{ N_t \sigma_x^2+\sigma_n^2}{2}   \right)
 }
\right)
$}  \ \text{[bpcu]}   \text{.}
\label{eq:I_analytical_short}
\end{equation}
For the case of perfect CSI it holds $\kappa=\frac{1}{2}$ and the variance term is equal to zero, which yields
\begin{equation}
\scalebox{0.99}{$
I_{\text{R}_{k}} = 
\frac{1}{2} \log_2 \left ( 1 +  \frac{  \sigma_x^2 
\left(1+\frac{\alpha}{2 N_r}\right)^2
N_r 
}{ \frac{\sigma_x^2}{2}
\delta_B
    (K-1)
+
\sigma_n^2 \delta_B 
+
2\frac{  \pi-2 }{\pi } \zeta^{-2} (1+\frac{\alpha}{2N_r})    
+2 \zeta^{-2} \delta_B
\left(
\frac{2}{\pi}
-  \zeta^2
\frac{ N_t \sigma_x^2+\sigma_n^2}{2}   \right)
 }
\right)
$}  \ \text{[bpcu]}   \text{.} \label{eq:I_analytical_short_perfect CSI}
\end{equation}
}

==> algorithm.tex <==
\begin{algorithm}
  \caption{Proposed DPA-IDD Algorithm}
	\label{alg:DPA_IDD}
  \begin{algorithmic}    %[1] %for numbers
    \State{Select one method for the extrinsic information computation}
    \State{Initialize $\boldsymbol{L}_a=\boldsymbol{0}$}
	\For{$j=1:N_{iter}-1$}
	\vspace{1mm}
	\For{$i=1:\frac{N_b}{R}$}
	\State{Using $\boldsymbol{L}_a$, compute $L_e(c_{k,i})$ according to the } 
	\State{method previously selected}
	\EndFor
	\State{Organize $\boldsymbol{L}_e=\pr{L_e(c_{k,1}), \hdots, L_e(c_{k,\frac{N_b}{R}})}^T$}
	\vspace{1mm}
	\State{Forward $\boldsymbol{L}_e$ to the message-passing decoder}
	\State{Using the decoder's output $\boldsymbol{L}$, update $\boldsymbol{L}_a=\boldsymbol{L}-\boldsymbol{L}_e$}
	\EndFor
	\For{$i=1:\frac{N_b}{R}$}
	\State{Using $\boldsymbol{L}_a$, compute $L_e(c_{k,i})$ according to the } 
	\State{method previously selected}
	\EndFor
	\State{Organize $\boldsymbol{L}_e=\pr{L_e(c_{k,1}), \hdots, L_e(c_{k,\frac{N_b}{R}})}^T$}
	\vspace{1mm}
	\State{Forward $\boldsymbol{L}_e$ to the message-passing decoder}
	\State{Using the decoder's output compute $\hat{\boldsymbol{c}_k}=-\frac{\text{sgn}\pc{\boldsymbol{L}-1}}{2}$}
	\State{Finally $\hat{\boldsymbol{m}}=\pr{c_{k, R N_b+1},\hdots,c_{k, \frac{N_b}{R}}}$ }
\end{algorithmic}
\end{algorithm}


==> tikzlibrarydsp.code.tex <==
% -------------------------------------------------------------------------
% This library for block diagrams and signal flow graphs was inspired by
% the library "signalflow" of Dr. Karlheinz Ochs, Ruhr-University of Bochum,
% Germany. Furthermore, some ideas were taken from the library "circuitikz"
% of Massimo A. Redaelli and from the PGF library itself.
%
% Copyright 2012 by Matthias Hotz
%
% This work is licensed under the Creative Commons Attribution 2.5 Generic
% License. To view a copy of this license, visit
%          http://creativecommons.org/licenses/by/2.5/
% or send a letter to Creative Commons, 444 Castro Street, Suite 900,
% Mountain View, California, 94041, USA.
% -------------------------------------------------------------------------

\usetikzlibrary{arrows, calc, positioning, decorations.markings}

% -------------------------------------------------------------------------
% Parameters for the library

\newcommand{\dsplinewidth}{0.25mm}           % Line width for connections
\newcommand{\dspblocklinewidth}{0.3mm}       % Line width for blocks
\newcommand{\dspoperatordiameter}{4mm}       % Diameter for adder, multiplier, mixer
\newcommand{\dspoperatorlabelspacing}{2mm}   % Distance from symbol to label for adder, multiplier, mixer
\newcommand{\dspnoderadius}{1mm}             % Filled and empty node
\newcommand{\dspsquareblocksize}{8mm}        % Size for square blocks, e.g. for delay elements, decimator, expander
\newcommand{\dspfilterwidth}{14mm}           % Width of a filter block

% -------------------------------------------------------------------------
% Define new arrow heads

\pgfarrowsdeclare{dsparrow}{dsparrow}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt} % Solid line (do not dash)
	\pgfsetmiterjoin	 % Fixed miter join of line
	\pgfsetbuttcap		 % Fixed butt cap of line
	\pgfpathmoveto{\pgfpoint{-4\arrowsize}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{4\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{-4\arrowsize}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

\pgfarrowsdeclare{dsparrowmid}{dsparrowmid}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt}
	\pgfsetmiterjoin
	\pgfsetbuttcap
	\pgfpathmoveto{\pgfpoint{0}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{8\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{0}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

% -------------------------------------------------------------------------
% Define new node shapes

\makeatletter

\pgfkeys{/tikz/dsp/label/.initial=above}

% Generic shape generator for operators, i.e. nodes with a circular
% shape with an additional customizable drawing and a text label
\long\def\dspdeclareoperator#1#2{
	\pgfdeclareshape{#1}
	{
		% Saved anchors, macros and dimensions
		\savedanchor\centerpoint{\pgfpointorigin}
		\savedmacro\label{\def\label{\pgfkeysvalueof{/tikz/dsp/label}}}
	  \saveddimen\radius
	  {
		  \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
		  \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
	    \ifdim\pgf@xa>\pgf@ya
	      \pgf@x=.5\pgf@xa
	    \else
	      \pgf@x=.5\pgf@ya
	    \fi
	  }
	  
	  % Inherit all anchors from the 'circle'-shape:
	  \inheritanchor[from={circle}]{center}
	  \inheritanchor[from={circle}]{mid}
	  \inheritanchor[from={circle}]{base}
	  \inheritanchor[from={circle}]{north}
	  \inheritanchor[from={circle}]{south}
	  \inheritanchor[from={circle}]{west}
	  \inheritanchor[from={circle}]{east}
	  \inheritanchor[from={circle}]{mid west}
	  \inheritanchor[from={circle}]{mid east}
	  \inheritanchor[from={circle}]{base west}
	  \inheritanchor[from={circle}]{base east}
	  \inheritanchor[from={circle}]{north west}
	  \inheritanchor[from={circle}]{south west}
	  \inheritanchor[from={circle}]{north east}
	  \inheritanchor[from={circle}]{south east}
	  \inheritanchorborder[from={circle}]
	  
	  % Draw circle and embed additional code
	  \backgroundpath
	  {
	    % Draw circle
	    \pgfpathcircle{\centerpoint}{\radius}
	    
	    % Embed additional code
	    % (Note that this code must call e.g. \pgfusepathqstroke
	    #2
	  }
	
		% Define anchor parametrized by the PGF key /tikz/dsp/label
	  \anchor{text}
	  {
			\centerpoint
			%
	    \def\templabelabove{above}
	    \def\templabelbelow{below}
	    \def\templabelleft{left}
	    \def\templabelright{right}
	    \pgfutil@tempdima=\dspoperatorlabelspacing
	    %
	    \ifx\label\templabelabove
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by \radius
				\advance\pgf@y by \pgfutil@tempdima
	    \fi
	    %
	    \ifx\label\templabelbelow
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by -\radius
				\advance\pgf@y by -\pgfutil@tempdima
				\advance\pgf@y by -\ht\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelleft
				\advance\pgf@x by -\radius
				\advance\pgf@x by -\pgfutil@tempdima
				\advance\pgf@x by -\wd\pgfnodeparttextbox
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelright
				\advance\pgf@x by \radius
				\advance\pgf@x by \pgfutil@tempdima
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	  }
	}
}

\dspdeclareoperator{dspshapecircle}{\pgfusepathqstroke}

\dspdeclareoperator{dspshapecirclefull}{\pgfusepathqfillstroke}

\dspdeclareoperator{dspshapeadder}{
	% Coordinate offset for the plus
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.55\pgfutil@tempdima
	
	% Draw plus
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{0pt}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{0pt}}}
	
	\pgfusepathqstroke
}

\dspdeclareoperator{dspshapemixer}{
	% Coordinate offset for the cross
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.707106781\pgfutil@tempdima
	
	% Draw cross
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{ \pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{-\pgfutil@tempdima}}}
	
	\pgfusepathqstroke
}

\makeatother

% -------------------------------------------------------------------------
% Define node styles

\tikzset{dspadder/.style={shape=dspshapeadder,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmultiplier/.style={shape=dspshapecircle,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmixer/.style={shape=dspshapemixer,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}

\tikzset{dspnodeopen/.style={shape=dspshapecircle,line width=\dsplinewidth,minimum size=\dspnoderadius}}
\tikzset{dspnodefull/.style={shape=dspshapecirclefull,line width=\dsplinewidth,fill,minimum size=\dspnoderadius}}

% The fixed specification of text height and text depth is the somewhat
% unaesthetic workaround to align the text in different node at the same
% baseline. See the PGF/TikZ manual, ch. 5.1.
\tikzset{dspsquare/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum size=\dspsquareblocksize}}
\tikzset{dspfilter/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum height=\dspsquareblocksize,minimum width=\dspfilterwidth}}

% -------------------------------------------------------------------------
% Define "signal flow" lines

\tikzset{dspline/.style={line width=\dsplinewidth},line cap=round,line join=round}
\tikzset{dspconn/.style={->,>=dsparrow,line width=\dsplinewidth},line cap=round,line join=round}%line cap=rect,line join=miter}
\tikzset{dspflow/.style={line width=\dsplinewidth,line cap=round,line join=round,
  decoration={markings,mark=at position 0.5 with {\arrow{dsparrowmid}}},postaction={decorate}}}

% -------------------------------------------------------------------------
% Define various utility macros

\newcommand{\downsamplertext}[1]{\raisebox{0.1em}{$\big\downarrow$}#1}
\newcommand{\upsamplertext}[1]{\raisebox{0.1em}{$\big\uparrow$}#1}

